Towards Fast, Flexible and Sensor-Free Control of Standalone PVDG Systems

In this thesis, the problem of fast, effective and low cost control of a Standalone Photovoltaic Distributed Generation (SPVDG) system is considered . On-site generation from these systems is more efficient when the power is transmitted via DC due to elimination of transmission losses and needless energy conversions. The inherent low-inertia of these systems added with fluctuation of output power and uncertain load consumption, calls for advanced control techniques to ensure fast and stable operation during various intermittencies. These techniques are expensive since they demand installation of many sophisticated sensors. The computation power provided by the fast growing IC technology can be utilized to estimate different parameters in a system and reduce the need for expensive sensing equipment. This work provides solutions to problems encountered in the development of faster, more stable and sensor-free voltage control and maximum power point tracking(MPPT) for SPVDG systems with PV and battery.

==> Content/certificate.tex <==
\makeatletter
\thispagestyle{plain}
\pagenumbering{roman}
\setcounter{page}{1}
\begin{center}
{\Large \textbf{Certificate}}
\end{center}
\vspace{2cm}
This is to certify that the work contained in the thesis entitled ``\textbf{Towards Fast, Flexible and Sensor-Free Control of Standalone PVDG Systems}'', by Meher Preetam Korukonda \vspace{1pt} (Roll No.\rollno), has been carried out under our supervision for the partial fulfillment of M.Tech degree in the \dept, IIT Kanpur and this work has not been submitted elsewhere for any other degree.

\vspace{3cm}


\hfill
\begin{minipage}{0.7\textwidth}

\begin{flushright}
\centering
\includegraphics[width=0.5\linewidth]{Figures/sirsign.png}\\
%\caption{Structure of SPVDG System}
%\label{fig:spvdg0}
\textbf{\supervisor}\\
\supervisorPosition\\
\dept\\
\IIT\\
\instaddress\\
\end{flushright}
\end{minipage}

\vspace{2cm}

\begin{minipage}{0.2\textwidth}
\begin{flushleft} 

\thesisdate % Some error is there 
\end{flushleft}
\end{minipage}
%\begin{flushright}
%\textbf{\supervicor}\\
%\supervicorPosition\\
%\dept\\
%\IIT\\
%\instaddress
%\end{flushright}


%\makeatother
